A New Benchmark For Evaluation Of Graph-Theoretic Algorithms

We propose a new graph-theoretic benchmark in this paper. The benchmark is developed to address shortcomings of an existing widely-used graph benchmark. We thoroughly studied a large number of traditional and contemporary graph algorithms reported in the literature to have clear understanding of their algorithmic and run-time characteristics. Based on this study, we designed a suite of kernels, each of which represents a specific class of graph algorithms. The kernels are designed to capture the typical run-time behavior of target algorithms accurately, while limiting computational and spatial overhead to ensure its computation finishes in reasonable time. We expect that the developed benchmark will serve as a much needed tool for evaluating different architectures and programming models to run graph algorithms.

==> kernel6.tex <==
\subsection{Kernel 6}
\begin{algorithm}[plain]
\caption{Kernel 6}
\label{kernel:6}
\begin{algorithmic}[1]
% generate a pattern
% insert a pattern into the graph OR select a pattern from existing 

\STATE Input:   Graph G(V, E), $\alpha$, and $m$ 
\STATE Output:  $k$, the number of clusters that maximizes objective function

\STATE Let G$^\prime$(V$^\prime$, E$^\prime$) be a graph, where
V$^\prime$ = $\{v\in$ V$\mid$ Color[$v$] $>\alpha\}$ and
E$^\prime$ = $\{e = (u, v, w)\in$E $\mid u, v \in$ V$\}$
\STATE $i \leftarrow 0$
\STATE $k \leftarrow 1$
\STATE $g_1 \leftarrow V^\prime$
\STATE $G_1 = \{g_1\}$
\WHILE{$i < m$}
\STATE $g_{min} \leftarrow g_j$ such that $g_j =  min_{g\in G_i}$ Density($g$)
\STATE $G_i \leftarrow G_i - g_{min}$
\STATE $g_{new} \leftarrow \emptyset$
\FORALL {$\forall v\in g_{min}$}
\STATE $g_{new} \leftarrow g_{new} \cup \{v\}$
\IF {Objective($G_i \cup g_{min}$) $>$ Objective($G_i \cup (g_{min} - \{v\}) \cup (g_{new} \cup \{v\})$)}
\STATE $g_{min} \leftarrow g_{min} - \{v\}$
\STATE $g_{new} \leftarrow g_{new} \cup \{v\}$
\ENDIF
\IF {$g_{new} = \emptyset$}
\STATE Stop
\ELSE
\STATE $G_i \leftarrow G_i \cup g_{min} \cup g_{new}$
\STATE $k \leftarrow k + 1$
\ENDIF
\ENDFOR
\STATE $i \leftarrow i + 1$
\ENDWHILE

\STATE \vspace{0pt}
\STATE {\bf function} Density($g$)
\STATE $S_i \leftarrow \{e = (u, v, w)\in E^\prime\mid u\in g$ and $v\in g\}$
\STATE $S_e \leftarrow \{e = (u, v, w)\in E^\prime\mid e\not\in S_i$ and $(u\in g$ or $v\in g)\}$
\STATE $d \leftarrow \frac{\mid S_i\mid}{\mid S_e\mid}$
\STATE {\bf end function}

\STATE \vspace{0pt}
\STATE {\bf function} Objective($G$)
\STATE return $\sum_{g\in G}$ H(Density($g$))
\STATE {\bf end function}

\STATE \vspace{0pt}
\STATE {\bf function} H($p$)
\STATE return $-p\cdot log_2 p - (1-p)\cdot log_2 (1-p)$
\STATE {\bf end function}

	\end{algorithmic}
	\end{algorithm}


	% ALGORITHM DESCRIPTION
	%	for faster generation
	%	degree calculation
%	weight and colors
%	parallelization


